Scalar Collapse in AdS

Recently, studies of the gravitational collapse of a scalar field within spherically symmetric AdS spacetimes was presented in \cite{Bizon:2011gg,Jalmuzna:2011qw} which showed an instability of pure AdS to black hole formation. In particular, the work showed that arbitrarily small initial configurations of scalar field evolved through some number of reflections off the AdS boundary until a black hole forms. We consider this same system, extended to include a complex scalar field, and reproduce this phenomena. We present tests of our numerical code that demonstrate convergence and consistency. We study the properties of the evolution as the scalar pulse becomes more compact examining the asymptotic behavior of the scalar field, an observable in the corresponding boundary CFT. We demonstrate that such BH formation occurs even when one places a reflecting boundary at finite radius indicating that the sharpening is a property of gravity in a bounded domain, not of AdS itself. We examine how the initial energy is transferred to higher frequencies --which leads to black hole formation-- and uncover interesting features of this transfer.

==> alex.tex <==
\catcode`\@=11

%%%
%%%%%% draftcontrol
%%%%%%%%%
\expandafter\ifx\csname draftcontrol\endcsname\relax\global\def\draftcontrol{0}
\fi

%%%
%%%%%% draftdate
%%%%%%%%%
{\count255=\time\divide\count255 by 60
\xdef\hourmin{\number\count255}
\multiply\count255 by-60\advance\count255 by\time
\xdef\hourmin{\hourmin:\ifnum\count255<10 0\fi\the\count255}}
\def\draftdate{\number\month/\number\day/\number\year\ \ \ \hourmin }

%%%
%%%%%% titlepage (adapted from article.cls)
%%%%%%%%%
\newcommand\makepapertitle{\par
  \begingroup
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
    \def\@makefnmark{\rlap{\@textsuperscript{\normalfont\@thefnmark}}}%
    \long\def\@makefntext##1{\parindent 1em\noindent
            \hb@xt@1.8em{%
                \hss\@textsuperscript{\normalfont\@thefnmark}}##1}%
     \newpage
     \global\@topnum\z@   % Prevents figures from going at top of page.
     \@makepapertitle
     \thispagestyle{empty}\@thanks
  \endgroup
  \setcounter{footnote}{0}%
  \global\let\thanks\relax
  \global\let\makepapertitle\relax
  \global\let\@makepapertitle\relax
  \global\let\@thanks\@empty
  \global\let\@author\@empty
  \global\let\@date\@empty
  \global\let\@title\@empty
  \global\let\title\relax
  \global\let\author\relax
  \global\let\date\relax
  \global\let\and\relax
  \def\version{\let\version\@version\@gobble}
}
\def\@makepapertitle{%
  \newpage
   \ifnum\draftcontrol=1 {}
   \version\versionno
   \vskip 3em%
   \else
   \hfill\hbox to 3cm {\parbox{4cm}{\@pubnum}\hss}%
   \vskip 3em%
   \fi
   \begin{center}%
   \let \footnote \thanks
     {\LARGE {\@title}}%
     \vskip 1.5em%
     {\normalsize%\large
       \lineskip .5em%
       \begin{tabular}[t]{c}%
         \@author
       \end{tabular}\par}%
     \vskip 1.5em%
     {\@bstract}%
     \end{center}%
     \vskip 1.5em
     \@date%
   \par
}

\gdef\@pubnum{}
%\@latex@error{No \noexpand \pubnum given}\@ehc}
\def\pubnum#1{%
  \gdef\@pubnum{#1}}

\gdef\@bstract{}
\def\Abstract#1{%
  \gdef\@bstract{%
   \parbox{\textwidth-0pc}{%
   \centerline{\bf Abstract}\penalty1000%
\kern.2cm%
\noindent%\abstractfont \baselineskip=12pt
\renewcommand\baselinestretch{1.0}%
{#1}}}
}


%%%
%%%%%% pagestyle
%%%%%%%%% for body of text
%%%%%%%%%%%%
\def\ps@paper{\let\@mkboth\@gobbletwo%
     \ifnum\draftcontrol=1
    \def\@oddfoot{\hbox to \textwidth{\tiny \versionno \hfil\tiny\draftdate}%
    \hskip -\textwidth \hbox to \textwidth{\hfil\rm\thepage\hfil}}%
     \else\def\@oddfoot{\hbox to \textwidth{\hfil\rm\thepage\hfil}}
     \fi
     \let\@evenfoot\@oddfoot
}
%%%%%%%%%%%%%%%%%%

%%%
%%%%%% front vs body vs coda
%%%%%%%%%
\def\body{\clearpage
%         \pagenumbering{arabic}
          \pagestyle{paper}
    }
\newenvironment{acknowledgments}{%
\vskip 3.25ex
%\@startsection {section}{1}{\z@}%
%                                   {-3.25ex \@plus -1ex \@minus -.2ex}%
%                                   {1.5ex \@plus.2ex}%
%                                   {\normalfont\normalsize\bfseries}
\noindent {\bf Acknowledgments}
%\vskip 0in
%\noindent
}

%%%%%%%%%%%%

%%%
%%%%%% definitions for draftmode
%%%%%%%%%
%%%%%%%%%%%% versioncontrol
%%%%%%%%%%%%%%%
\def\@version#1{\ifnum\draftcontrol=1
\typeout{}\typeout{#1}\typeout{}
\vskip3mm\centerline{\hbox{\fbox{\normalsize{\tt DRAFT -- #1 -- }
                   {\draftdate}}}}\vskip3mm
\fi}
\let\version\@version
%%%%%%%%%%%% labels in math mode
%%%%%%%%%%%%%%%
\long\def\eqlabel#1{\ifnum\draftcontrol=1
                    \tag@false  % there are some problems with multline without this
                    \tag*{(\theequation) \hbox to -0.2cm{\hspace{0cm}\small{#1}\hss}}
                    \refstepcounter{equation}
                    \edef\@currentlabel{\theequation}
                    \ltx@label{#1}          % use old LaTeX \label instead of new definition
                                            % of \label in AMSLaTeX.
                    \else
                    \label{#1}
                    \fi
                    }
%%%%%%%%%%%% citations keys in bibliography (very short version of showkeys.sty)
%%%%%%%%%%%%%%%
\let\st@bibitem\@bibitem
\let\st@lbibitem\@lbibitem
\ifnum\draftcontrol=1
  \def\@bibitem#1{%
    \st@bibitem{#1}\a@@label{#1}\ignorespaces}
  \def\@lbibitem[#1]#2{%
    \st@lbibitem[#1]{#2}\a@@label{#2}\ignorespaces}
  \def\a@@label#1{%
    \gdef\a@lab{\smash{\normalfont\small#1}}
    \ifvmode
      \if@inlabel
        \global\setbox\@labels\hbox{%
          \llap{\a@lab\let\a@lab\relax
                \kern\@totalleftmargin\kern\marginparsep}%
          \box\@labels}%
      \fi
    \fi}
\fi
%%%%%%%%%%%%%%%



